Experimental and Phenomenological Investigations of the MiniBooNE Anomaly

This thesis covers a range of experimental and theoretical efforts to elucidate the origin of the $4.8\sigma$ MiniBooNE low energy excess (LEE). We begin with the follow-up MicroBooNE experiment, which took data along the BNB from 2016 to 2021. This thesis specifically presents MicroBooNE's search for $\nu_e$ charged-current quasi-elastic (CCQE) interactions consistent with two-body scattering. The two-body CCQE analysis uses a novel reconstruction process, including a number of deep-learning-based algorithms, to isolate a sample of $\nu_e$ CCQE interaction candidates with $75\%$ purity. The analysis rules out an entirely $\nu_e$-based explanation of the MiniBooNE excess at the $2.4\sigma$ confidence level. We next perform a combined fit of MicroBooNE and MiniBooNE data to the popular $3+1$ model; even after the MicroBooNE results, allowed regions in $\Delta m^2$-$\sin^2 2_{\theta_{\mu e}}$ parameter space exist at the $3\sigma$ confidence level. This thesis also demonstrates that the MicroBooNE data are consistent with a $\overline{\nu}_e$-based explanation of the MiniBooNE LEE at the $<2\sigma$ confidence level. Next, we investigate a phenomenological explanation of the MiniBooNE excess combining the $3+1$ model with a dipole-coupled heavy neutral lepton (HNL). It is shown that a 500 MeV HNL can accommodate the energy and angular distributions of the LEE at the $2\sigma$ confidence level while avoiding stringent constraints derived from MINER$\nu$A elastic scattering data. Finally, we discuss the Coherent CAPTAIN-Mills experiment--a 10-ton light-based liquid argon detector at Los Alamos National Laboratory. The background rejection achieved from a novel Cherenkov-based reconstruction algorithm will enable world-leading sensitivity to a number of beyond-the-Standard Model physics scenarios, including dipole-coupled HNLs.

==> templates/READMEs/README_bibliography.tex <==
%% This file gives an overview on what you will need to do to create a
%% bibliographic database for references, as well as create the actual
%% bibliography for your thesis.

%% You should not need to touch the file biblio.tex.  This merely tells
%% latex to look for the file with the bibliographic info.  The file you
%% want to edit is main.bib.  For each entry, use the appropriate style
%% as designated in the file.

%% Citing your references:

%% When you cite a reference, you need to use the ``key'' you declare in
%% main.bib for the entry.  No one ever sees the keys, but you'll want to
%% use something you will easily remember.  For instance, if you had an
%% entry with:

%% 	   key=geer1

%% Then you would use \cite{geer1} to reference it within your thesis.

%% NOTE: You can not include references in your bibliography that are
%% never cited in your paper by default. If you need to do this, create a
%% key for the entry and at the end of your thesis include the line:

%% \nocite{key}

%% This should be done for every entry which is not explicitly cited.



==> templates/READMEs/README_main.tex <==
%% This file explains the options available to you for editing the file
%% main.tex.

%% The commands in this file allow you to specify options such as
%% spacing, double-sided printing, a draft copy, etc.   By default, 12pt
%% and lgrind are included; lgrind is the 2e style for including code in
%% your thesis.

%% \documentclass[12pt]{mitthesis}
%% \usepackage{lgrind}
%% \pagestyle{plain}

%% You can add options in the documentclass line as follows:

%% 	o  singlespace
%% 	\documentclass[12pt,singlespace]{mitthesis}
	
%% 	o  twoside
%% 	\documentclass[12pt,twoside]{mitthesis}

%% 	o  draft   (make sure to change the pagestyle to drafthead as well)
%% 	\documentclass[12pt,draft]{mitthesis}
%% 	\usepackage{lgrind}
%% 	\pagestyle{drafthead}

%% 	o vi   (for course vi and course viii theses)
%% 	\documentclass[12pt,vi]{mitthesis}

%% Any options you would use for report.sty will work here as well.


%% You should not need to change the first three lines and last two lines
%% below.  Be sure to include an \include command for each file you are
%% including in your thesis.
  
%% \include{cover}
%% \pagestyle{plain}
%% \include{contents}
%% \include{chap1}
%% \include{chap2}
%% \appendix
%% \include{appa}
%% \include{appb}
%% \include{biblio}
%% \end{document}

%% Comment: to include appendices use a single \appendix command followed 
%% by a number of \include{} commands as many files as needed, each of 
%% which should contain a \chapter{} command for the appendix title.


==> templates/READMEs/README_text.tex <==
%% This file includes the basic commands you will need to use within each
%% chapter of your thesis.

%% The file chap1.tex is a sample first chapter.  To get started, you may
%% just want to replace the text and commands in that file as needed.  In
%% general though, for each new chapter you want to do the following:

%% 	o Make sure the name has the extension .tex .  Otherwise, you
%% 	can call it anything you want.  For ease of use, all the
%% 	examples use chap1, chap2, etc.

%% 	o Add a line to the file main.tex that reads:
%% 	\include{yourfilename}

%% 	This should not include the .tex extension, because latex
%% 	assumes that is there.

%% Basic syntax:

%% 	o The first line of each chapter should be:
%% 	\chapter{Chapter Title}

%% 	o To start a new section (labeled chap#.sec# -- as in 1.1,
%% 	1.2, etc):
%% 	\section{Section Heading}

%% 	You can also include subsections:
%% 	\subsection{Heading}



